Channel Sounding for the Masses: Low Complexity GNU 802.11b Channel Impulse Response Estimation

New techniques in cross-layer wireless networks are building demand for ubiquitous channel sounding, that is, the capability to measure channel impulse response (CIR) with any standard wireless network and node. Towards that goal, we present a software-defined IEEE 802.11b receiver and CIR estimation system with little additional computational complexity compared to 802.11b reception alone. The system implementation, using the universal software radio peripheral (USRP) and GNU Radio, is described and compared to previous work. By overcoming computational limitations and performing direct-sequence spread-spectrum (DS-SS) matched filtering on the USRP, we enable high-quality yet inexpensive CIR estimation. We validate the channel sounder and present a drive test campaign which measures hundreds of channels between WiFi access points and an in-vehicle receiver in urban and suburban areas.

==> conc.tex <==
\section{Conclusion} \label{S:conc}

Future wireless networks are envisioned that rely on the real-time
estimation of CIR from received WiFi
packets for the purposes of cross-layer security, localization, and
environmental imaging. We present a CIR estimation system using an
inexpensive and open source hardware and software platform to enable
these emerging areas of research.  We show how accurate CIR estimation
can be performed using a resource-constrained FPGA, which provides a
proof-of-concept for future commercial devices. A deconvolution
algorithm is implemented to refine CIR estimates, and measurements
using known channels are conducted to verify estimator accuracy.  A
drive test is performed, recording CIR in six
different areas in a city, as an example of the use of the CIR
estimation system.

As an open source platform, others may improve upon the work described here.  As of the submission date, our implementation and source code have been downloaded at least 430 times since its first posting in March, 2008, not counting those downloads from hosts other than our own.  Work remains to additionally implement 802.11 transmission, in addition to reception and CIR estimation, on future devices, for example, on the USRP 2.0.  In general, the additional capability of the USRP 2.0 allows implementation of other transceiver features in addition to the CIR estimation described here.  Future work will also address  MIMO CIR estimation, using a bank of synchronized software radios.  Low complexity MIMO channel sounding will likely benefit the development of future cross-layer techniques in multiple-antenna wireless networks.



==> header.tex <==
\newcommand{\dd}[1]{{\tfrac{\partial}{\partial #1}}}
\newcommand{\dfd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dtwod}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\dtwodd}[2]{\frac{\partial^2}{\partial #1 \partial #2}}
\newcommand{\dndd}[3]{\frac{\partial^{#3}}{\partial {#1} \cdots \partial {#2}}}
\newcommand{\dtwofdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\Var}[2]{\mbox{Var}_{#1}\left[ {#2} \right]}
\newcommand{\Cov}[1]{\mbox{Cov}\left( {#1} \right)}
\newcommand{\E}[2]{E_{#1}\left[ {#2} \right]}
\newcommand{\I}[1]{\mathrm{I}_{#1}}
\newcommand{\PR}[1]{P\left[{#1}\right]}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}
%\nonumber\newcommand{\RE}{1}{{\mathbb{Re}\left\{#1\right\}}}
\newcommand{\argmin}[1]{\mathop{\mbox{argmin}}_{#1}}
\newcommand{\argmax}[1]{\mathop{\mbox{argmax}}_{#1}}
\newcommand{\argminX}{\argmin{ X: \; X^TX=I_D}}
\newcommand{\Order}[1]{\mathcal{O}\left( {#1} \right)}
\newcommand{\ds}[1]{\mathrm{d}{#1}}
\newcommand{\dv}[1]{\mathrm{d}\Vc{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\me}{\mathrm{e}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\vone}{\Vc{1}}
\newcommand{\vzero}{\Vc{0}}
\newcommand{\vI}{\Vc{I}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\diag}[1]{{\mbox{diag}\left\{{#1}\right\}}}
\newcommand{\bb}[0]{\bar{b}}
\newcommand{\bs}[0]{\bar{\sigma}}
\newcommand{\mbA}[0]{\mathbf{A}}
\newcommand{\mbB}[0]{\mathbf{B}}
\newcommand{\mbC}[0]{\mathbf{C}}
\newcommand{\mbD}[0]{\mathbf{D}}
\newcommand{\mbE}[0]{\mathbf{E}}
\newcommand{\mbF}[0]{\mathbf{F}}
\newcommand{\mbG}[0]{\mathbf{G}}
\newcommand{\mbH}[0]{\mathbf{H}}
\newcommand{\mbI}[0]{\mathbf{I}}
\newcommand{\mbJ}[0]{\mathbf{J}}
\newcommand{\mbK}[0]{\mathbf{K}}
\newcommand{\mbL}[0]{\mathbf{L}}
\newcommand{\mbM}[0]{\mathbf{M}}
\newcommand{\mbN}[0]{\mathbf{N}}
\newcommand{\mbO}[0]{\mathbf{O}}
\newcommand{\mbP}[0]{\mathbf{P}}
\newcommand{\mbQ}[0]{\mathbf{Q}}
\newcommand{\mbR}[0]{\mathbf{R}}
\newcommand{\mbS}[0]{\mathbf{S}}
\newcommand{\mbT}[0]{\mathbf{T}}
\newcommand{\mbU}[0]{\mathbf{U}}
\newcommand{\mbV}[0]{\mathbf{V}}
\newcommand{\mbW}[0]{\mathbf{W}}
\newcommand{\mbX}[0]{\mathbf{X}}
\newcommand{\mbY}[0]{\mathbf{Y}}
\newcommand{\mbZ}[0]{\mathbf{Z}}
\newcommand{\mba}[0]{\mathbf{a}}
\newcommand{\mbb}[0]{\mathbf{b}}
\newcommand{\mbc}[0]{\mathbf{c}}
\newcommand{\mbd}[0]{\mathbf{d}}
\newcommand{\mbe}[0]{\mathbf{e}}
\newcommand{\mbf}[0]{\mathbf{f}}
\newcommand{\mbg}[0]{\mathbf{g}}
\newcommand{\mbh}[0]{\mathbf{h}}
\newcommand{\mbi}[0]{\mathbf{i}}
\newcommand{\mbj}[0]{\mathbf{j}}
\newcommand{\mbk}[0]{\mathbf{k}}
\newcommand{\mbl}[0]{\mathbf{l}}
\newcommand{\mbm}[0]{\mathbf{m}}
\newcommand{\mbn}[0]{\mathbf{n}}
\newcommand{\mbo}[0]{\mathbf{o}}
\newcommand{\mbp}[0]{\mathbf{p}}
\newcommand{\mbq}[0]{\mathbf{q}}
\newcommand{\mbr}[0]{\mathbf{r}}
\newcommand{\mbs}[0]{\mathbf{s}}
\newcommand{\mbt}[0]{\mathbf{t}}
\newcommand{\mbu}[0]{\mathbf{u}}
\newcommand{\mbv}[0]{\mathbf{v}}
\newcommand{\mbtv}[0]{\mathbf{\tilde{v}}}
\newcommand{\mbw}[0]{\mathbf{w}}
\newcommand{\mbx}[0]{\mathbf{x}}
\newcommand{\mby}[0]{\mathbf{y}}
\newcommand{\mbty}[0]{\mathbf{\tilde{y}}}
\newcommand{\mbz}[0]{\mathbf{z}}
\newcommand{\mbzero}[0]{\mathbf{0}}
\newcommand{\mbalpha}[0]{{\boldsymbol{\alpha}}}
\newcommand{\mbdelta}[0]{{\boldsymbol{\delta}}}
\newcommand{\mbepsilon}[0]{{\boldsymbol{\epsilon}}}
\newcommand{\mbmu}[0]{{\boldsymbol{\mu}}}
\newcommand{\mbPi}[0]{{\boldsymbol{\Pi}}}
\newcommand{\mbpi}[0]{{\boldsymbol{\pi}}}
\newcommand{\mbtheta}[0]{{\boldsymbol{\theta}}}
\newcommand{\mbphi}[0]{{\boldsymbol{\phi}}}


\newcommand{\Definition}[2]{\vspace{0.1in} \noindent    {\begin{minipage}{\linewidth}\underline{\bf Def'n:}  {\it #1}\\
#2\end{minipage}}\vspace{0.1in} \\ }
\newcommand{\Lemma}[2]{\vspace{0.1in}\\ \noindent  {\begin{minipage}{\linewidth}\underline{\bf Lemma:}  {#1}\\
{\bf Proof:} #2 \end{minipage}}\vspace{0.1in} \\ }
\newcommand{\Theorem}[2]{\vspace{0.1in} \noindent \begin{minipage}{\linewidth}\underline{\bf Theorem:}
{#1} \\ {\bf Proof:} {#2} \end{minipage}\vspace{0.1in} \\ }
\newcommand{\StartOf}[1]{{\noindent \rule{\linewidth}{1pt}\\ \noindent \large \bf #1}\\}
\newcommand{\Today}[1]{{\noindent \large Today: #1}\\}
\newcommand{\Example}[1]{{\vspace{0.15in} \noindent \bf Example: #1}\\}
\newcommand{\Note}[1]{{\vspace{0.05in} \noindent {\bf Note:} #1}\\}
\newcommand{\IF}[1]{\,\,\,\, \mbox{if} \,\,\, #1}
\newcommand{\pdfarray}[2]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ 0, & o.w. \end{array}\right. }}
\newcommand{\pdfarrays}[4]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ {#3}, & {#4} \\ 0, & o.w. \end{array}\right. }}
\newcommand{\twooptions}[4]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ {#3}, & {#4} \end{array}\right. }}
\newcommand{\CDFarrays}[4]{{ \left\{\begin{array}{ll}
   0,    & {#3} < {#2} \\
   {#1}, & {#2} \le {#3} < {#4} \\
   1, & {#3} \ge {#4} \end{array}\right. }}
\newcommand{\CDFarray}[3]{{ \left\{\begin{array}{ll}
   0,    & {#3} < {#2} \\
   {#1}, & {#3} \ge {#2} \end{array}\right. }}
\newcommand{\CCDFarrays}[4]{{ \left\{\begin{array}{ll}
   1,    & {#3} < {#2} \\
   {#1}, & {#2} \le {#3} < {#4} \\
   0, & {#3} \ge {#4} \end{array}\right. }}
\newcommand{\CCDFarray}[3]{{ \left\{\begin{array}{ll}
   1,    & {#3} < {#2} \\
   {#1}, & {#3} \ge {#2} \end{array}\right. }}
\newcommand{\Vector}[1]{\left[ \begin{array}{c} #1 \end{array} \right]}
\newcommand{\MatTwoCols}[1]{\left[ \begin{array}{cc} #1 \end{array} \right]}
\newcommand{\MatThreeCols}[1]{\left[ \begin{array}{ccc} #1 \end{array} \right]}
\newcommand{\PP}[0]{\vspace{0.11in}\noindent}
\newcommand{\Fourier}[1]{{\mathfrak{F}\left\{ {#1}\right\}} }
\newcommand{\IFourier}[1]{{\mathfrak{F}^{-1}\left\{ {#1}\right\}} }
\newcommand{\DTFT}[1]{{\mathrm{DTFT}\left\{ {#1}\right\}} }
\newcommand{\IDTFT}[1]{{\mathrm{DTFT}^{-1}\left\{ {#1}\right\}} }
\newcommand{\rect}[0]{\mbox{rect}}
\newcommand{\sinc}[0]{\mbox{sinc}}
\newcommand{\Summary}[1]{{\vspace{0.15in} \noindent \bf Summary of today's lecture}: #1\\}
\newcommand{\rank}[0]{\mbox{rank}}
\newcommand{\atantwo}[2]{{\mbox{atan2} \left({#1}, {#2} \right) }}
\newcommand{\erf}[0]{\mbox{erf}}
\newcommand{\erfc}[0]{\mbox{erfc}}

\newcommand{\En}[0]{\mathcal{E}}
\newcommand{\Ebno}[0]{\frac{\mathcal{E}_b}{N_0}}
\newcommand{\Question}[0]{{\vspace{0.15in} \noindent \bf Question:  }}
\newcommand{\dB}[0]{\mbox{(dB)}}
\newcommand{\dBm}[0]{\mbox{(dBm)}}
\newcommand{\dBW}[0]{\mbox{(dBW)}}
\newcommand{\intinfty}[2]{{\int_{#1 = -\infty}^{\infty} #2  d{#1} }}
\newcommand{\decision}[2]{{{#1 \atop >} \atop {< \atop #2}}}
\newcommand{\Q}[1]{{\mbox{Q}\left( {#1} \right)}}
\newcommand{\Qinv}[1]{{\mbox{Q}^{-1}\left( {#1} \right)}}
\newcommand{\sgn}[1]{{\mbox{sgn}\left\{ {#1} \right\}}}
\newcommand{\entropy}[1]{H\left[ {#1} \right]}
\newcommand{\stdPM}[0]{(P,\mathcal{F}, \Omega)}
\newcommand{\apriori}[0]{\emph{a priori} }
\newcommand{\nnn}[0]{\nonumber \\ }
\newcommand{\nn}[0]{\nonumber }
\newcommand{\sifi}[0]{$\sigma$-field}
\newcommand{\communicateswith}[0]{{\leftrightarrow }}
\newcommand{\MatFourCols}[1]{\left[ \begin{array}{cccc} #1 \end{array} \right]}
\newcommand{\MatFiveCols}[1]{\left[ \begin{array}{ccccc} #1 \end{array} \right]}
\newcommand{\MatSixCols}[1]{\left[ \begin{array}{cccccc} #1 \end{array} \right]}
\newcommand{\MatSevenCols}[1]{\left[ \begin{array}{ccccccc} #1 \end{array} \right]}
\newcommand{\MatEightCols}[1]{\left[ \begin{array}{cccccccc} #1 \end{array} \right]}
\newcommand{\MatNineCols}[1]{\left[ \begin{array}{ccccccccc} #1 \end{array} \right]}
\newcommand{\limin}[1]{\lim_{{#1}\rightarrow \infty}}

